CICERO: A Dataset for Contextualized Commonsense Inference in Dialogues

This paper addresses the problem of dialogue reasoning with contextualized commonsense inference. We curate CICERO, a dataset of dyadic conversations with five types of utterance-level reasoning-based inferences: cause, subsequent event, prerequisite, motivation, and emotional reaction. The dataset contains 53,105 of such inferences from 5,672 dialogues. We use this dataset to solve relevant generative and discriminative tasks: generation of cause and subsequent event; generation of prerequisite, motivation, and listener's emotional reaction; and selection of plausible alternatives. Our results ascertain the value of such dialogue-centric commonsense knowledge datasets. It is our hope that CICERO will open new research avenues into commonsense-based dialogue reasoning.

==> causal_qa_results.tex <==
\begin{table}[t]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
\textbf{Model} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{BLEURT} & \textbf{BERTScore} \\
\midrule
\textbf{(i) Cause} & & \\
\quad T5 Large &  &  &  &  &  \\
\quad BART Large &  &  &  &  &  \\
\midrule
\textbf{(ii) Effect Full} & & \\
\quad T5 Large &  &  &  &  &  \\
\quad BART Large &  &  &  &  &  \\
\midrule
\textbf{(iii) Effect Clipped} & & \\
\quad T5 Large &  &  &  &  &  \\
\quad BART Large &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\caption{\footnotesize Results for Dialogue Causal Question Answering.}
\label{tab:cqa}
\end{table}

==> chained_cause_effect_results.tex <==
\begin{table}[t]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
\textbf{Model} & \textbf{BLEU2} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{CIDEr} & \textbf{Sem-Sim} \\
\midrule
\colorbox{almond}{\textbf{(1.1.4) Chained Cause}} & & \\
\quad \quad \code{T5}    & 	 0.1566   & 	0.1675  & 	 0.2757  & 	 0.5303  & 	 0.6518 \\
\quad \quad \code{GLUCOSE-T5}    &	0.1600  &	\bf 0.1697  &	\bf 0.2796  &	\bf 0.5633  &	\bf 0.6557\\
\cmidrule{2-6}
\colorbox{almond}{\textbf{(1.1.1)* Cause}} & & \\
\quad \quad \code{T5}   & 	 0.1503   & 	 0.1635  & 	 0.2634  &  0.4591  & 0.6284  \\
\quad \quad \code{GLUCOSE-T5}     &	\bf 0.1564  &	\bf 0.1636  &	\bf 0.2709  &	\bf 0.4915  &	\bf 0.6310\\
\midrule
\colorbox{ghostwhite}{\textbf{(1.1.5) Chained SE}} & & \\
\quad \quad \code{T5}   & 	 \textbf{0.1813}   & 	 \textbf{0.1784}  & 	 0.2940  & 	 0.5136  & 	 0.6469 \\
\quad \quad \code{GLUCOSE-T5}    &	0.1789  &	0.1776  &	\bf 0.2943  &	\bf 0.5218  &	\bf 0.6516\\
\cmidrule{2-6}
\colorbox{ghostwhite}{\textbf{(1.1.2)* SE}} & & \\
\quad \quad \code{T5}   & 	 \bf 0.1622  & 	 0.0841   & 	 0.2764  & 	 0.4167  & 0.6279  \\
\quad \quad \code{GLUCOSE-T5}    &	0.1612  &	\bf 0.1628  &	\bf 0.2778  &	\bf 0.4471  &	\bf 0.6294\\
\bottomrule
\end{tabular}
}
\caption{\footnotesize Results of the \dataset{}$_{NLG}$ subtasks -- chained cause and subsequent event generation. (1.1.1)* and (1.1.2)* indicates results from Task 1.1.1 and 1.1.2 (as in \cref{tab:results}), but only for targets which have both cause and effect annotated, ensuring a fair comparison with (1.1.4) and (1.1.5). \colorbox{ghostwhite}{SE} denotes Subsequent Event.}
\label{tab:cqa}
\end{table}

==> dataset_comparison.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|ccccc|c}
\toprule
\textbf{Dataset} & \textbf{Extractive} & \textbf{Speculative} & \textbf{CSK} & \textbf{Background Knowledge} & \textbf{Contextual Inference} \\
\midrule

CIDER & \cellcolor{Green2} Yes & \cellcolor{Gray1} No & \cellcolor{Green2} Yes & \cellcolor{Green2} Yes & \cellcolor{Green2} Yes\\
\hl{CIDER2} & & & & & \\
\hl{CIDER2} & & & & & \\

\bottomrule
\end{tabular}
}
\caption{}
\label{tab:comparison}
\end{table*}

==> listener_reaction_results.tex <==
\begin{table}[t]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
\textbf{Model} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{BLEURT} & \textbf{BERTScore} \\
\midrule
T5 Large &  &  &  &  &  \\
BART Large &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\caption{\footnotesize Results for Listener Emotional Response Generation.}
\label{tab:lerg}
\end{table}

==> mcq_examples.tex <==
\begin{table}[h]
  \centering
  \begin{subtable}{0.95\linewidth}
   \small
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{p{10cm}}
    \toprule
    \textbf{A \pmb {($u_1$)}}: Hi, Jenny. Is it true you're moving to London?
    \textbf{B \pmb {($u_2$)}}: Yes, it is.
    \textbf{A \pmb {($u_3$)}}: What made you decide to do that?
    \textbf{B \pmb {($u_4$)}}: Work, mainly. I'm sure I'll be able to find a job there.
    \textbf{A \pmb {($u_5$)}}: You're probably right. But where are you going to live?
    \textbf{B \pmb {($u_6$)}}: I hope I'll find a flat to share with somebody. That way it will be cheaper.
    \textbf{A \pmb {($u_7$)}}: Yes, that's a good idea. Are you taking your dog with you?
    \textbf{B \pmb {($u_8$)}}:  No, I don't think so. My parents have offered to take care of him, and I don't think he'd be happy in the city.
    \textbf{A \pmb {($u_9$)}}: You're probably right. But aren't you afraid of moving to such a big place, especially after living in a small village?
    \textbf{B \pmb {($u_{10}$)}}: Not really. I think I'll enjoy myself. There's so much to do there; I expect I won't miss the countryside much and I can always come back and visit. 
    \textbf{A \pmb {($u_{11}$)}}: Well, I just hope you'll invite me to stay when you get settled.
    \textbf{B \pmb {($u_{12}$)}}:  Of course I will.
    \\
    \end{tabular}
    }
\end{subtable}
\bigskip
\begin{subtable}{\linewidth}
 \small
\centering
\resizebox{0.95\linewidth}{!}{
  \begin{tabular}{p{10cm}}
      \toprule
      \textbf{Target -} \pmb{$u_6$}; \textbf{Inference:} \colorbox{almond}{\bf Cause}; \textbf{Annotation:}  Being an expensive city, it is quite difficult to find an affordable place to live in London. \\
      \midrule
      \textbf{Target -} \pmb{$u_{10}$}; \textbf{Inference:} \colorbox{almond}{\bf Cause}; \textbf{Annotation:} Jinny realizes that a city like London will provide a great quality of life for her. \\
      
      \midrule
      \textbf{Target -} \pmb{$u_6$}; \textbf{Inference:} \colorbox{ghostwhite}{\bf Effect}; \textbf{Annotation:}  The listener gives an idea to Jenny to find the flat on some online portal for searching flatmates as well plenty of cheaper options. \\
      
      \midrule
      \textbf{Target -} \pmb{$u_{10}$}; \textbf{Inference:} \colorbox{ghostwhite}{\bf Effect}; \textbf{Annotation:}  Jenny inquired a social club in London and ask for their membership to utilize her free time. \\
      
      \midrule
      \textbf{Target -} \pmb{$u_4$}; \textbf{Inference:} \colorbox{Green2}{\bf Prerequisite}; \textbf{Annotation:}  Jenny has completed her studies. \\
      \midrule
      \textbf{Target -} \pmb{$u_{12}$}; \textbf{Inference:} \colorbox{Green2}{\bf Prerequisite}; \textbf{Annotation:}  Jenny and the listener are good friends. \\
      
      \midrule
      \textbf{Target -} \pmb{$u_6$}; \textbf{Inference:} \colorbox{Blue2}{\bf Motivation}; \textbf{Annotation:}  Jenny is optimistic about having someone as her flatmate to save rent. \\
      
      \midrule
      \textbf{Target -} \pmb{$u_{12}$}; \textbf{Inference:} \colorbox{Gray3}{\bf Reaction}; \textbf{Annotation:}  The listener is happy for Jenny and looks forward to being invited to London by Jenny. \\
      \bottomrule
  \end{tabular}
  }
\end{subtable}
\caption{}
\label{tab:mcq-examples}
\end{table}

==> prompt_results.tex <==
\begin{table}[t]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
\textbf{Model} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{METEOR} & \textbf{BLEURT} & \textbf{BERTScore} \\
\midrule
\textbf{Cause} & & \\
\quad T5 Large &  &  &  &  &  \\
\quad BART Large &  &  &  &  &  \\
\midrule
\textbf{Effect} & & \\
\quad T5 Large &  &  &  &  &  \\
\quad BART Large &  &  &  &  &  \\
\midrule
\textbf{Prerequisite} & & \\
\quad T5 Large &  &  &  &  &  \\
\quad BART Large &  &  &  &  &  \\
\midrule
\textbf{Motivation} & & \\
\quad T5 Large &  &  &  &  &  \\
\quad BART Large &  &  &  &  &  \\
\midrule
\textbf{Reaction} & & \\
\quad T5 Large &  &  &  &  &  \\
\quad BART Large &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\caption{\footnotesize Results for Prompt based Commonsense Generation.}
\label{tab:prompt}
\end{table}
